Client-side Active Measurements Without Application Control

Monitoring performance and availability are critical to operating successful content provider networks. Internet measurements provide data needed for traffic engineering, alerting, and network diagnostics. While there are significant benefits to combining server-side passive measurements with end-user active measurements, these capabilities are limited to a small number of content providers with both network and application control. In this work, we present a solution to a long-standing problem for a method to issue active measurements from clients without application control. Our approach uses features of the W3C Network Error Logging specification that allow a CDN to induce a browser connection to an HTTPS server of the CDN's choosing.

==> headers-json.tex <==
\begin{Verbatim}[commandchars=\\\{\},frame=leftline,framesep=1.5ex,framerule=0.8pt,fontsize=\smaller]
\PY{p}{N}\PY{p}{E}\PY{p}{L}\PY{p}{:} \PY{p}{\PYZob{}}\PY{n+nt}{\PYZdq{}report\PYZus{}to\PYZdq{}}\PY{p}{:} \PY{l+s+s2}{\PYZdq{}default\PYZdq{}}\PY{p}{,} \PY{n+nt}{\PYZdq{}max\PYZus{}age\PYZdq{}}\PY{p}{:} \PY{l+m+mi}{43200}\PY{p}{,} 
      \PY{n+nt}{\PYZdq{}success\PYZus{}fraction\PYZdq{}}\PY{p}{:} \PY{l+m+mf}{0.25}\PY{p}{,} \PY{n+nt}{\PYZdq{}failure\PYZus{}fraction\PYZdq{}}\PY{p}{:} \PY{l+m+mf}{1.0}\PY{p}{\PYZcb{}}
     
\PY{p}{R}\PY{p}{e}\PY{p}{p}\PY{p}{o}\PY{p}{r}\PY{p}{t}\PY{p}{\PYZhy{}}\PY{p}{T}\PY{p}{o}\PY{p}{:} \PY{p}{\PYZob{}}\PY{n+nt}{\PYZdq{}group\PYZdq{}}\PY{p}{:} \PY{l+s+s2}{\PYZdq{}default\PYZdq{}}\PY{p}{,} \PY{n+nt}{\PYZdq{}max\PYZus{}age\PYZdq{}}\PY{p}{:} \PY{l+m+mi}{86400}\PY{p}{,} 
     \PY{n+nt}{\PYZdq{}endpoints\PYZdq{}}\PY{p}{:} \PY{p}{[}\PY{p}{\PYZob{}}\PY{n+nt}{\PYZdq{}url\PYZdq{}}\PY{p}{:} \PY{l+s+s2}{\PYZdq{}https://neltest.com/report\PYZdq{}}\PY{p}{\PYZcb{}}\PY{p}{]}\PY{p}{\PYZcb{}}
\end{Verbatim}


==> nel.tex <==
\section{Network Error Logging}
\label{sec:nel}

Network Error Logging (\nel) is a W3C specification~\cite{nelspec} for reporting client-side networking errors in web applications to help developers and operators detect and mitigate availability issues. \nel enables a content provider to install a measurement policy for a domain by setting the \nelheader and \reportheader headers in the HTTP response as shown in Listing~\ref{listing:nelheaders}. In this example, the \nelheader header specifies a policy to sample 25\% of successful requests and 100\% of failed requests and is valid for 24 hours (43200 seconds). Once the policy is installed, it applies to all resources from the same domain, and optionally sub-domain, for the \texttt{max\_age} duration. The \reportheader header's \texttt{endpoints} field is a list of \textit{report endpoints} where the browser will upload reports in a background process after a short delay, outside of the browser's critical rendering path. If the first endpoint is unreachable, the browser retries on subsequent endpoints.

\begin{listing}[ht]
\inputminted[fontsize=\footnotesize]{python}{headers.json}
\vspace{-5pt}
\caption{Example \nel and Report-To response headers used to configure a measurement policy with JSON. These headers can be set by the server for a web resource (e.g. GET path/pic.jpg).}
\label{listing:nelheaders}
\end{listing}

\NEL's first public release was in September 2018 in Chrome 69\footnote{At the time of this writing, the request\_header and response\_header features remain disabled in Chrome due to privacy concerns.}. Other browsers based on Chromium, such as Microsoft Edge (79+), inherit \nel functionality. 

\matt{mentioned same origin policy}

\footnote{View installed }





==> related.tex <==
\section{Related Work}
\label{sec:related}


